Early Validation of Cyber-Physical Space Systems via Multi-Concerns Integration

Cyber-physical space systems are engineered systems operating within physical space with design requirements that depend on space, e.g., regarding location or movement behavior. They are built from and depend upon the seamless integration of computation and physical components. Typical examples include systems where software-driven agents such as mobile robots explore space and perform actions to complete particular missions. Design of such a system often depends on multiple concerns expressed by different stakeholders, capturing different aspects of the system. We propose a model-driven approach supporting (a) separation of concerns during design, (b) systematic and semi-automatic integration of separately modeled concerns, and finally (c) early validation via statistical model checking. We evaluate our approach over two different case studies of cyber-physical space systems.

==> letter.tex <==

\begin{center}
\Large{\textbf{Response to decision letter}}\\
\vspace{0.5cm}
\large{\textbf{JSS-D-19-00936 -- ``Early validation of CPSS via Multi-Concerns Integration''}}
\end{center}

\vspace{1cm}

\noindent
Dear Prof. Mirandola,
\\
\\
We thank the anonymous reviewers for the detailed, useful feedback and suggestions, which were
instrumental to improve the manuscript. 
\vspace{0.5cm}

\noindent
In the following, we report on reviewers' comments. Each of them is followed by our explanation as well as an indication of the corresponding changes in the manuscript. 
\\

 \noindent  Kind regards,\\
\vspace{0.1cm}

\noindent
    Nianyu Li\\
    Christos Tsigkanos\\
    Zhi Jin\\
   Zhenjiang Hu\\
    Carlo Ghezzi

\newpage



\section*{Review 2}


\textbf{Comment \#1.} 
The authors motivated in a convincing way the absence of the missing experiment and I think it is sufficient. However, some previous comments have not been addressed (not even in the response letter), and so I report them below together with some other minor observations.
\begin{lquote}
We are thankful for the detailed comments, which were addressed in the manuscript.
\end{lquote}



\textbf{Comment \#1.} 
- page 11, line 3 after listing 1
"HA or HB. From location HB"
There is no location "HB" in Fig. 3. There is RA and HA.
\begin{lquote}
Fixed.
\end{lquote}

\textbf{Comment \#2.} 
- page 12, Section 5.1, after definition of $\phi$
"d is a integer"
Since it is about time, I think that "d" must be a non-negative integer. See, e.g., Sect. 2
\begin{lquote}
Fixed.
\end{lquote}

\textbf{Comment \#3.} 
- page 14, last but one line
"in such cases a single ..."
This has been just said in the previous paragraph ("a single robot has no chance ..."). It should be removed or merged.
\begin{lquote}
The sentence was removed as it indeed was a repetition.
\end{lquote}

\textbf{Comment \#4.} 
- page 14, footnote 2
I would use reference [52] has done in other parts of the paper.
\begin{lquote}
Fixed.
\end{lquote}

\textbf{Comment \#5.} 
- page 15, line 4
"grid"
Can there be obstacles in the grid?
\begin{lquote}
In the scenario considered, passive objects such as obstacles are ignored.
\end{lquote}

\textbf{Comment \#6.} 
- page 17, last two lines
"In Figure 7, ... is more evident ..."
I still believe that the advantage is not so visible from the figure. I would use a different type of figure: for each UAV number, I would make a figure with both the plots of Bluetooth and ZigBee. Therefore, there should be three figures. If the authors don't want to make three figures (and keep these two), the interval on the y-axis should be the same (going from 0 to 0.8).
\begin{lquote}
The latter suggestion was implemented. Specifically, the interval on the y-axes of Fig.7 are the same, showing probabilities of adoption of Bluetooth and ZigBee.
\end{lquote}


\textbf{Comment \#7.} 
- Typos -
\begin{lquote}
We are grateful for the detailed typos inspection -- they were fixed accordingly.
\end{lquote}




==> relwork.tex <==
%!TEX root = ../paper.tex

% \vspace{-0.4cm}
%\vspace{-0.2cm}

\section{Related Work}
\label{sec:relWork}
% \vspace{-0.1cm}

% \begin{shaded}
% Section 5 discusses related work in statistical model checking while using sight of the main issues raised, that is the modelling and verification of space-dependent systems. As a result, some relevant references such as Tsigkanos et al. ESEC/FSE 2017 are missing.
% \end{shaded}
%\sherry{model composition part missing}




%In this paper, we elaborated on the previous work ~\cite{smcworkshop,fse17} and focused on modeling and early validation of CPSS. We presented an integrated framework that supports modeling via separation of concerns and model analysis via statistical model checking. We can classify related work into two categories. 
%Firstly, we consider model integration with separation of concerns, positioning our work. Then, we discuss validation for cyber-physical systems, particularly about SMC in recent literature. The objective is not to be exhaustive, but to position our work with respect to relevant lines of research followed by larger research communities. 
%Thereafter, we enumerate several applications of the SMC within cyber-physical space systems.


%-Related work on model composition.

%\sherry{Find other approaches where they work with state machines in a more or less similar way. Check Uchitel et al, synthesis works too where they do synthesis from state machines and mention them too }

The evolutionary and interactive nature of CPSS aims at building cross-domain intelligence in heterogenous and dynamic environment~\cite{DBLP:journals/percom/WuKT11}. 
Crosscutting problems can be observed at scenario modeling level where one model may present several tangled concerns, compromising requirements and system evolution. It is desirable to analyze how the crosscutting scenarios interact with other scenarios at early stages of software development~\cite{DBLP:books/daglib/0032906}. To achieve the modularization, separation of concerns are not enough to construct complex software systems and efficient model composition or integration mechanisms should be supported with minimum effort~\cite{SoCOO}.  
%Building up a comprehensive model of the system could also benefit from the application of the approach that allows model composition with crosscutting concerns or aspects~\cite{DBLP:journals/pieee/AkkayaDEL16}. 


A two-hemisphere modeling approach has been put up to automate the process of class diagram development (target composed model) and enable knowledge representation in terms of business process model and concept model~\cite{DBLP:conf/caise/NikiforovaK04}.  Service composition techniques have been extended for CPSS, and developed PE-ontology and PE-SOA model to connect physical entities and service specifications respectively~\cite{DBLP:conf/icsoft/2017}. 
Besides, synthesis of behavioural models for modeling and reasoning about system behavior at the architectural level, such as labelled transition system and modal transition system, from scenario-based specifications has been extensively studied~\cite{DBLP:phd/ethos/Uchitel03,DBLP:journals/tse/SibayBUK13}. 
In our work, the SoC is maintained at the automaton level by deriving separately automata from domain applications or domain knowledge.
Previous work~\cite{fse17} has targeted automatically obtaining automata structures for cyber-physical spaces, which can bootstrap a core aspect of the present work -- behaviour STAs from space descriptions. Moreover, physical models may be automatically obtained~\cite{tsigkanos2016architecting,sescps}. Grounding our approach on MDE principles and standards facilitates development of integrated and open tool environments for systematic model-based engineering~\cite{gam,DBLP:journals/pieee/SztipanovitsBKL18} on top of physical space domain models. 


\begin{shaded}
Given the ever increasing integration and the inherent uncertainties CPS face, the metaphor of agents and multi-agent systems (MAS) still matches and principles from MAS remain particularly attractive for engineering cyber-physical systems today~\cite{DBLP:conf/emas/MascardiW18}. 
An agent-oriented approach based on the agent-based cooperating smart object (ACOSO) has been investigated to provide agent design and programming models for the actual construction of a cyber-physical IoT system~\cite{DBLP:journals/tsmc/FortinoRSSZ18}. Architecture-based design of MAS puts architecture at the center of the development activities, documenting specific concerns such as roles, organizations, and interaction protocols, applying to automated guided vehicles and transportation systems~\cite{Weyns2010}. Supporting cooperation and coordination across entities and agents enables the constituting elements to work together effectively~\cite{DBLP:journals/cii/LeitaoCK16}, which is similarly one of the concerns in this paper. However, to the best of our knowledge, although such works propose agent-oriented solutions for modelling, simulating and analyzing CPS, they do not emphasize separation of concerns nor modeling  their automatic integration. 


The operating environment is %\sherry{remove broadly}
recognized as a first-class entity within multi-agent systems, since it mediates interactions between agents and their access to resources~\cite{DBLP:journals/aamas/WeynsOO07}.  Ferber et al integrate the environment into an Agent-Group-Role model and consider social and physical embedding as different kinds of modes, such as the role in a group or the way perceiving and acting within a space, for an agent to manifest itself~\cite{DBLP:conf/e4mas/FerberMB04}. Using appropriate ontologies offering richer and more expressive presentation is another key aspect in the design of environment~\cite{DBLP:journals/jaihc/DuricRCSJ19}. 
Agent environments are essential for multi-agent systems. 
%\christos{the next sentence contradicts the first sentence of the paragraph}
However, most works do not integrate the agents' environment as a primary modeling abstraction~\cite{DBLP:conf/e4mas/WeynsM14}. In contrast, we explicitly model the spatial environment as a state-transition structure -- instead of the modes or ontologies in other work -- and consider the possible spatial behavior of active agents as a special concern in our model integration approach. 
\end{shaded}
%\christos{what are "modes"?}\sherry{I give more details on the related work section}



%Statistical model checking has emerged as a compromise between verification and testing, where statistical techniques produce an estimate for a system's satisfaction of a property~\cite{larsen2014statistical} while being competitive with state of the art numerical solution methods for probabilistic model checking~\cite{younes2005verification,DBLP:conf/isola/GrosuPRSSY14}. The modeling discipline utilizing timed automata with different types of relationships among clocks of a distributed system~\cite{rodriguez2013using} inspire the modeling of different activities in our approach. Subsequently, statistical methods~\cite{younes2005verification} (e.g. hypothesis testing or Monte Carlo simulation) upon execution traces, produce statistical quantitative evidence about the system's satisfaction or violation of a requirements specification~\cite{sen2004statistical}. Similarly to our approach, high-level constructs for communication and data propagation, explicitly taking into account stochastics are developed for validation of cyber-physical multi-agent systems~\cite{kroiss2016logic}. Statistical model checking has been used to support design of systems-of-systems, such as smart cities and internet-of-things, i.e. for quantifying mission achievement~\cite{arnold2016application} or reasoning in smart grids~\cite{yuksel2012modelling}. 


% \sherry{is this paragraph all about interaction???}
% This paper established the foundation for statistical probabilistic model checking,
% an approach to probabilistic model checking based on hypothesis testing and
% simulation. And they demonstrate that this approach is competitive with state-of-
% the-art numerical solution methods for probabilistic model checking.~\cite{younes2005verification}
% The paper focuses on the system which is unknown and passively observed to
% obtain sample traces but cannot be controlled. Given a set of executions (obtained
% by Monte Carlo simulation) and a property, the algorithm in the paper checks, based
% on statistical hypothesis testing, whether the sample provides evidence to conclude
% the satisfaction or violation of a property, and computes a quantitative measure (p-
% value of the tests) of confidence in its answer. In our paper, we use this method
% generating execution traces upon which statistical methods produce statistical
% evidence about the system’s satisfaction or violation of a requirements specification.\cite{sen2004statistical}.
% They use SMC to estimate the probability with which the property holds on the system and develop a distributed SMC tool.\cite{kyle2015statistical}.
% From the applications perspective, research in diverse areas has considered analyses of space-dependent systems.%; we discuss key relevant approaches.




Notable recent approaches have focused on applications of the statistical model checking paradigm in diverse domains within cyber-physical space systems.
Statistical model checking and spatio-temporal logics are combined to tackle problems in collective and smart transportation systems, allowing estimation of likelihood of specific spatio-temporal predicates such as clusters in space~\cite{ciancia2016tool}.
%Our approach utilizes automata obtained from space models given in a domain-specific notation, abstracted into a formally defined static and discrete topological model, upon which dynamic topological changes are modeled by transformation rules~\cite{fse17,tdscpreprint}; spatial behavioral models are then automatically derived. Advanced spatial predication could be added to our model support~\cite{ciancia2015spatio}, something we identify as future work. 
In~\cite{ruijters2016better}, a framework utilizing statistical model checking for dependability within railway systems is developed. 
Rare events problems in cyber physical space applications have been emphasized in statistical model checking, either by adding feedback control to efficiently estimate the probability~\cite{DBLP:conf/isola/KalajdzicJLBLSG16}, by importance sampling and Cross-Entropy method~\cite{DBLP:conf/atva/ClarkeZ11}, or by importance splitting and reformulating the rare probability~\cite{DBLP:conf/cav/JegourelLS13}.
Also within software engineering, the ActivFORMS~\cite{deltaiot} framework exploits statistical model checking at runtime to select configurations that comply with self-adaptation goals over an internet-of-things network topology. In contrast, our approach targets early requirements validation through separation of system design concerns.
% In\cite{david2015statistical}, analysis of biological systems is targetted, along with integration with domain specific tools and formalisms specifically tailored towards the biology domain.



% Engineering Trustworthy Self-Adaptive Software with Dynamic Assurance Cases~\cite{calinescu2017engineering}





% Timed Automata
% - Rajeev Alur, David L. Dill: A Theory of Timed Automata. Theor. Comput. Sci.
% 126(2): 183-235 (1994)\cite{alur1994theory}
% % Abstract : We propose timed (finite) automata to model the behavior of real-time
% % systems over time. Our definition provides a simple, and yet powerful, way to
% % annotate state-transition graphs with timing constraints using finitely many real-
% % valued clocks. A timed automaton accepts timed words-infinite sequences in which a
% % real-valued time of occurrence is associated with each symbol. We study timed
% % automata from the perspective of formal language theory: we consider closure
% % properties, decision problems, and subclasses. We consider both nondeterministic
% % and deterministic transition structures, and both Büchi and Muller acceptance
% % conditions. We show that nondeterministic timed automata are closed under union
% % and intersection, but not under complementation, whereas deterministic timed Muller
% % automata are closed under all Boolean operations.
% % - Paritosh K. Pandya, P. Vijay Suman: An Introduction to Timed Automata. Modern
% % Applications of Automata Theory 2012: 111-148
% % Abstract : Timed automata have emerged as a prominent model for representation
% % and analysis of real-time systems. The study of closure properties and decision
% % problems for timed automata provides key insights into their computational power.
% % The resulting algorithms have influenced the development of automatic analysis
% % tools for model checking real-time systems. In this chapter we provide an
% % introduction to the theory of timed automata.
% % - Guillermo Rodríguez-Navas, Julian Proenza:
% % Using Timed Automata for Modeling Distributed Systems with Clocks: Challenges
% % and Solutions. IEEE Trans. Software Eng. 39(6): 857-868 (2013)
% % Abstract : The application of model checking for the formal verification of distributed
% % embedded systems requires the adoption of techniques for realistically modeling the
% % temporal behavior of such systems. This paper discusses how to model with timed
% % automata the different types of relationships that may be found among the computer
% % clocks of a distributed system, namely, ideal clocks, drifting clocks, and synchronized
% % clocks. For each kind of relationship, a suitable modeling pattern is thoroughly
% % described and formally verified.
% % 1Monday, 16 October 2017
% % SMC
% - H. L. S. Younes. Verification and Planning for Stochastic Processes with
% Asynchronous Events. PhD thesis, Carnegie Mellon, 2005 \cite{younes2005verification}
% % Abstract : We consider a general model of stochastic discrete event systems with
% % asynchronous events, and propose to develop efficient algorithms for verification
% % and control of such systems.
% - Koushik Sen, Mahesh Viswanathan, and Gul Agha. Statistical model checking of
% black-box probabilistic systems. In CAV, LNCS 3114, pages 202–215. Springer,
% 2004 \cite{sen2004statistical}
% % Abstract : We propose a new statistical approach to analyzing stochastic systems
% % against specifications given in a sublogic of continuous stochastic logic (CSL).
% % Unlike past numerical and statistical analysis methods, we assume that the system
% % under investigation is an unknown, deployed black-box that can be passively
% % observed to obtain sample traces, but cannot be controlled. Given a set of
% % executions (obtained by Monte Carlo simulation) and a property, our algorithm
% % checks, based on statistical hypothesis testing, whether the sample provides
% % evidence to conclude the satisfaction or violation of a property, and computes a
% % quantitative measure (p-value of the tests) of confidence in its answer; if the sample
% % does not provide statistical evidence to conclude the satisfaction or violation of the
% % property, the algorithm may respond with a “don’t know” answer.
% - Kim G. Larsen, Axel Legay: Statistical Model Checking: Past, Present, and
% Future. ISoLA (1) 2016: 3-15 \cite{larsen2014statisticalb}
% % Abstract : Statistical Model Checking (SMC) is a compromise between verification
% % and testing where executions of the systems are monitored until an algorithm from
% % statistics can produce an estimate for the system to satisfy a given property.
% % The objective of this introduction is to summarizes SMC as well as a series of
% % challenges for which contributors at Isola propose a solution.


